Glance: Accelerating Diffusion Models with 1 Sample

Diffusion models have achieved remarkable success in image generation, yet their deployment remains constrained by the heavy computational cost and the need for numerous inference steps. Previous efforts on fewer-step distillation attempt to skip redundant steps by training compact student models, yet they often suffer from heavy retraining costs and degraded generalization. In this work, we take a different perspective: we accelerate smartly, not evenly, applying smaller speedups to early semantic stages and larger ones to later redundant phases. We instantiate this phase-aware strategy with two experts that specialize in slow and fast denoising phases. Surprisingly, instead of investing massive effort in retraining student models, we find that simply equipping the base model with lightweight LoRA adapters achieves both efficient acceleration and strong generalization. We refer to these two adapters as Slow-LoRA and Fast-LoRA. Through extensive experiments, our method achieves up to 5 acceleration over the base model while maintaining comparable visual quality across diverse benchmarks. Remarkably, the LoRA experts are trained with only 1 samples on a single V100 within one hour, yet the resulting models generalize strongly on unseen prompts.

==> sec/1_introduction_alex.tex <==
\section{Introduction}
\label{sec:intro}


\input{Figures/tex/figure3}

\input{Figures/tex/figure1}


Diffusion and flow matching models \cite{sohl2015deep,ho2020denoising,song2019generative,lipman2022flow,albergo2022building} have shown strong capabilities in generating high-fidelity images, marking a significant advancement in the field of generative modeling. 
Despite their impressive performance, a notable challenge is the \textbf{high inference cost} due to its iterative denoising nature, 50 steps in natural.
For example, we experimentally find that Qwen-image takes 1 hour to generate only 1 sample in 1 V100 GPU.
It is straightforward to raise a question: can we use these solid models with "cheap" solution?

To address this issue, various methods are proposed to accelerate the sampling process of diffusion models, including improving the efficiency of samplers \cite{karras2022elucidating,lu2022dpm,lu2022dpm_p,liu2022pseudo} and employing model distillation techniques \cite{salimans2022progressive,liu2022flow,frans2024one,song2023consistency,kim2023consistency,geng2025mean} to reduce the number of inference steps. 
Recent advancements in trajectory distillation methods and distribution matching techniques \cite{yin2024one,yin2024improved,sauer2024adversarial,zhou2024score}, often enhanced by adversarial learning at scale, have shown considerable promise in generating high-fidelity images in extremely low steps such as one to four steps.
often makes such distilled model tuning approach less feasible. 
Unfortuntatly, these ''expensive'' methods require massive tuning time and collect a huge number of training sample.
(cf., 3840 A100 GPU hours for SDXL-DMD2 \cite{yin2024improved} and 3072 A100 GPU hours for Qwen-Image-Lightning \cite{ModelTC2025QwenImageLightning})
These methods far away from the "cheap" motivation.


In this work, we try to challenge this stable point and  train the model with 1 sample.
Specifically, we take a different perspective by revisiting the denoising dynamics of diffusion models. 
We observe that the generation trajectory consists of two qualitatively distinct phases: an early semantic phase that determines global structure, and a late redundant phase that primarily refines texture. 
Uniform acceleration treats all steps equally, yet semantic steps are far more sensitive to perturbation than redundant ones. 
This motivates a phase-aware acceleration strategy that applies small speedups to semantic steps and large speedups to redundant steps.

To realize this idea, we introduce \ours, implemented as a pair of lightweight LoRA adapters that attach to the pretrained diffusion model. 
Slow-LoRA stabilizes early semantic formation, while Fast-LoRA accelerates late-stage refinement. 
Crucially, our method does not require training a new student network and the base model remains unchanged. 
Both LoRA experts are trained using only \textbf{one sample} on a single V100 GPU within \textbf{one hour} (Fig.~\ref{fig:introduction}). 

To demonstrate its scalability, we distill FLUX.1-12B \cite{flux2024} and Qwen-Image-20B \cite{wu2025qwenimagetechnicalreport} text-to-image models into 8- and 10-step students, respectively.
Extensive experiments across six text-to-image benchmarks show that \ours exhibits performance curves that closely track those of the base models, indicating strong consistency under accelerated inference. 
On OneIG-Bench, HPSv2, and GenEval, the performance of \ours reaches \textbf{92.60\%}, \textbf{99.67\%}, and \textbf{96.71\%} of the teacher models, respectively. 
We further conduct dense ablation studies on slow–fast phase decomposition, timestep allocation, and training data scaling, all of which consistently validate the effectiveness and robustness of our design.

We summarize the contributions as follows: 
% % (1) We employ a phase-aware acceleration scheme that treats semantic and redundant steps differently for a more natural and stable speedup.
% (2) We introduce Slow-LoRA and Fast-LoRA, two lightweight adapters that plug into the base model, enabling effective phase-wise acceleration with only one sample and one hour of training.
%
% (3) \ours achieves a \textbf{5$\times$ speed-up} over FLUX.1 and Qwen-Image while retaining teacher-level performance across six benchmarks.

\begin{itemize}

    \item 
    We employ a phase-aware acceleration scheme that treats semantic and redundant steps differently for a more natural and stable speedup.
    
    \item 
    We introduce two lightweight adapters that plug into the base model, enabling effective acceleration with only one sample and one hour of training.

    \item 
    \ours achieves a \textbf{5$\times$ speed-up} over FLUX.1 and Qwen-Image while retaining teacher-level performance across six benchmarks.

\end{itemize}

\input{Figures/tex/figure2}




